Active Learning for Rapid Targeted Synthesis of Compositionally Complex Alloys

The next generation of advanced materials is tending toward increasingly complex compositions. Synthesizing precise composition is time-consuming and becomes exponentially demanding with increasing compositional complexity. An experienced human operator does significantly better than a beginner but still struggles to consistently achieve precision when synthesis parameters are coupled. The time to optimize synthesis becomes a barrier to exploring scientifically and technologically exciting compositionally complex materials. This investigation demonstrates an Active Learning (AL) approach for optimizing physical vapor deposition synthesis of thin-film alloys with up to five principal elements. We compared AL based on Gaussian Process (GP) and Random Forest (RF) models. The best performing models were able to discover synthesis parameters for a target quinary alloy in 14 iterations. We also demonstrate the capability of these models to be used in transfer learning tasks. RF and GP models trained on lower dimensional systems (i.e. ternary, quarternary) show an immediate improvement in prediction accuracy compared to models trained only on quinary samples. Furthermore, samples that only share a few elements in common with the target composition can be used for model pre-training. We believe that such AL approaches can be widely adapted to significantly accelerate the exploration of compositionally complex materials.

==> stream_of_consciousness.tex <==
Several laboratories across the world are using combinatorial synthesis to search for new types of materials. Examples can include solar cells, perovskites, structural alloys, thermoelectrics, cathode materials, bulk metallic glasses, rare earth free permanent magnets, and more. 

These high throughput studies often require a lot of time in the laboratory tuning manufacturign processes. One manufacturing process that is commonly used for combinatorial synthesis is magnetron sputtering, a physical vapor deposition process. I will insert citations here that point to these studies. 

Manufacturing a thin film requires finding the right settings for your physical vapor deposition system in order to get the right composition. You have to tune the power of the sputtering gun, or its angle relative to the substrate, to get the deposition rate correctly. This requires calibrating the deposition rate of each individual element you are sputtering. However, knowing the sputtering rate of a single element isn't enough. When multiple guns are sputtering at once they interact and impact the sputtering rates of the other guns, meaning the calibration you did is only so good.

So what scientists have to do is artistically iterate through many differnet sputtering gun parameters (power, angles) until they find the right composition. This iterative process is time confusing and often frustrating. 

We have used an active learning approach to speed up the process of finding optimal manufacturing parameters for a given target composition.

First, the sputtering system we are using is an AJA International Orion ATC. It can sputter up to 5 elements at a time on either DC or RF cathodes. There are two important input settings for each gun: the power of the gun (in watts) and its arc length (in mm) relative to the position of the substrate. (Reference the first figure here that shows the sputtering system we use.)

First we combine these two descriptors into a single descriptor that we call the normalized energy. It is dimensionless. The normalized energy is equal to the Power divided by the arc length multiplied by 6. Write an equation that expresses this.

Once we have normalized our inputs we use the modAL python package to do active learning. We use modAL in combination with several sklearn regression functions. In particular we tried out several ensemble decision tree models and several gaussian process regression models with different kernels. The model takes as input a vector of length 6, one entry for each element in the sputtering system. It predicts a value y, which is also a vector of length six. The contents of y are the atomic percents of each element in the thin film sample.

We start by randomly sampling our dataset for 5 initial training points. Then we query each learner for the next training point to test in the set. We choose the next training point based on the maximum uncertainty of the predictions. 

You can see the performance of each model in total prediction error in a (reference the second figure here). The Random forest ensemble model performed the best and was able to get a prediction accuracy within 5% after only 40 samples. This is in contrast to the 60 attempts that it took a human using the intution method.

You can also see the prediction error of each element in (reference the third figure here). Ti, which was the dopant element for all systems, has the lowest prediction error. It also has the lowest variance both in terms of input values and output values. Sb had the worst performance across all elements. This is likely becaues of the impact of sputtering Ta; when the Ta gun is off, the sputtering rate of Sb is high. When Ta is on, the sputtering rate of Sb drops significantly. The model was not able to distinguish well between these two modes.

We also demonstrate the ability of the model to provide interpretable results to the users. It is not enough to simply have a high prediction error. We also want the user to be able to get out what manufacturing parameters (power and angle) that they should use to achieve a given composition.  To do this, we created a grid of points consisting of different powers and angles. The grid of points only lies within the range of current powers and angles in our training dataset. We trained the model on an initial 5 data points as before. We then query the model and ask what sample to learn enxt. After teaching the model the new sample, we make a prediction on the grid of points. We see whether or not the target value is in the list of predicted values. We do this by taking hte log likelihood of the predicted values and the target values. If the log likelihood is less than 1, then we say it is a match. We then look at the power and angles associated with that value and see if it is near the real value used to make the target value.

(insert a reference to the the final figure here). You can see that after only 5 iterations the model is able to predict the target composition to within 1% accuracy. Furthermore, we were also able to get the proper power and angle needed to manufacture a sample with this composition.

We believe this can be a powerful tool for any scientists doing combinatorial thin film sputtering. We strongly enocurage you to set up an active learnign appraoch and use it to guide your synthesis of compositionally complex systems."

Take everything that I just wrote and generate a first draft in LaTeX. Use proper, scientific language. Try to write as complete of a draft as possible. I will fill it in with a literature review, citations, and figures.
